Distributed Optimal Control of Graph Symmetric Systems via Graph Filters

Designing distributed optimal controllers subject to communication constraints is a difficult problem unless structural assumptions are imposed on the underlying dynamics and information exchange structure, e.g., sparsity, delay, or spatial invariance. In this paper, we borrow ideas from graph signal processing and define and analyze a class of Graph Symmetric Systems (GSSs), which are systems that are symmetric with respect to an underlying graph topology. We show that for linear quadratic problems subject to dynamics defined by a GSS, the optimal centralized controller is given by a novel class of graph filters with transfer function valued filter taps and can be implemented via distributed message passing. We then propose several methods for approximating the optimal centralized graph filter by a distributed controller only requiring communication with a small subset of neighboring subsystems. We further provide stability and suboptimality guarantees for the resulting distributed controllers. Finally, we empirically demonstrate that our approach allows for a principled tradeoff between communication cost and performance while guaranteeing stability. Our results can be viewed as a first step towards bridging the fields of distributed optimal control and graph signal processing.

==> texFiles/oldProblemFormulation.tex <==
\section{The Distributed Linear-Quadratic Problem} \label{sec:LQR}

Consider a linear system described by a state vector $x(t) \in \fdR^{N}$ and controlled by an action $u(t) \in \fdR^{N}$.
The system is determined by the system matrix $A \in \fdR^{N \times N}$ and the control matrix  $B \in \fdR^{N \times N}$ as follows:
% eq:linearDynamics
\begin{equation} \label{eq:linearDynamics}
    x(t+1) = A \vcx(t) + B \vcu(t) + w(t)
\end{equation}
%
for $t=0,1,\ldots$ and where $\{w(t)\}$ is a random, white noise sequence.
\red{FG: If we include the noise, isn't it a `LQG' problem?}
The linear-quadratic problem consists on finding the \red{static} state-feedback controller $K:\fdR^{N} \to \fdR^{N}$ that minimizes a given quadratic cost
% eq:quadraticCost
\begin{equation} \label{eq:quadraticCost}
    \fnJ \big( \{x(t)\}, \{u(t)\} \big) = \lim_{T \to \infty} \sum_{t=0}^{T-1} \xp_{w} \big[ x(t)^{\Tr} Q x(t) + u(t)^{\Tr} R u(t) \big]
\end{equation}
%
where $u(t) = K(x(t))$ and where $Q, R \in \fdR^{N \times N}$ are known symmetric matrices that satisfy $Q \succeq 0$ and $R \succ 0$.
The controller that solves
% eq:LQG
\begin{equation} \label{eq:LQG}
    \min_{\fnH \in \fdH} \fnJ\big( \{\vcx(t)\},\{\vcu(t)\} \big) \quad \text{s. t. } \vcu(t) = \fnH\big(\vcx(t)\big)
\end{equation}
%
is a linear static controller $\vcu(t) = \mtH^{\opt} \vcx(t)$ with linear operator $\mtH^{\opt} = -(\mtR+ \mtB^{\Tr} \mtP \mtB)^{-1}\mtB^{\Tr} \mtP \mtA$ and where $\mtP$ is a matrix obtained as the unique solution to the following discrete-time algebraic Ricatti equation:
% eq:Ricatti
\begin{equation} \label{eq:Ricatti}
    \mtP = \mtA^{\Tr} \mtP \mtA - \mtA^{\Tr} \mtP \mtB \big( \mtR+ \mtB^{\Tr} \mtP \mtB \big)^{-1} \mtB^{\Tr} \mtP \mtA + \mtQ.
\end{equation}
%

Consider now a linear system of interconnected components described by a graph $\graph = \{\stV, \stE\}$, where $\stV = \{\lmv_{1},\ldots,\lmv_{N}\}$ is the set of $N$ components (nodes) and where $\stE \subseteq \stV \times \stV$ is the set of the corresponding interconnections (edges).
It is assumed that the graph is undirected, i.e. $(\lmv_{i},\lmv_{j}) \in \stE$ if and only if $(\lmv_{j},\lmv_{i}) \in \stE$.
In this context, the state vector $\vcx(t)$ is such that the $i^{\text{th}}$ entry $[\vcx(t)]_{i} = x_{i}(t)$ corresponds to the value of the state at the  $i^{\text{th}}$ component $\lmv_{i}$ at time $t$.
Likewise, the $i^{\text{th}}$ entry of the control action $[\vcu(t)]_{i} = u_{i}(t)$ corresponds to the action taken by the $i^{\text{th}}$ component at time $t$.

Controlling systems of interconnected components oftentimes demands distributed controllers.
These are controllers $\fnH_{\stG}:\fdR^{N} \to \fdR^{N}$ whose operations are restricted to follow the connection patterns of the system.
That is, the only operations allowed are those that involve components that share a connection.
This is denoted by the subscript $\stG$ in the controller notation $\fnH_{\stG}$,  indicating that a distributed controller has to respect the structure of the graph $\stG$ describing the connections between components.

A convenient way to be able to define operations that respect the graph structure is to leverage a graph matrix description (GMD) $\mtS \in \fdR^{N \times N}$.
The matrix $\mtS$ is such that the $(i,j)^{\text{th}}$ entry is zero whenever there is no connection between components $\lmv_{i}$ and $\lmv_{j}$, i.e. $[\mtS]_{ij}=0$ if $i \neq j $ and $(\lmv_{i},\lmv_{j}) \notin \stE$.
Note that, since the graph is undirected, the matrix $\mtS$ is symmetric.
Therefore, it has en eigedecomposition in terms of an orthonormal basis of eigenvectors $\mtS = \mtV \mtLambda_{S} \mtV^{\Tr}$ where $\mtLambda_{S} \in \fdR^{N \times N}$ is a diagonal matrix with elements $\lambda_{S,i} \in \fdR$ such that $\mtS \vcv_{i} = \lambda_{S,i} \vcv_{i}$ for $\vcv_{i} \in \fdR^{N}$ being the $i^{\text{th}}$ column of $\mtV$.

In a general linear system as in \eqref{eq:linearDynamics}, the matrices $\mtA$ and $\mtB$ are not related to the structure of the underlying graph.
This means that the evolution of the system is not tied to the structure of connections, i.e. the vector $\vcx(t+1)$ can be built by linear combinations of the entries in $\vcx(t)$ that may not respect the interconnected nature of the system.
To be able to describe distributed, linear system dynamics, the GMD $\mtS$ has to be leveraged.
More specifically, we define a distributed linear system as follows:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%           Definition
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% def:distributedLinear
\begin{definition}[Distributed Linear System] \label{def:distributedLinear}
    Given a GMD $\mtS=\mtV \mtLambda_{S} \mtV^{\Tr}$, a linear system as in \eqref{eq:linearDynamics} is distributed if the system and control matrices satisfy
    % eq:distributedLinear
    \begin{equation} \label{eq:distributedLinear}
        \mtA = \mtV \mtLambda_{A} \mtV^{\Tr} \quad , \quad \mtB = \mtV \mtLambda_{B} \mtV^{\Tr}.
    \end{equation}
    %
\end{definition}
%
%%%%       End of Definition
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Def.~\ref{def:distributedLinear} requires that both the system matrix $\mtA$ and the control matrix $\mtB$ be simultaneously diagonalizable with the GMD $\mtS$.
In practical terms (for finite graphs with GMDs that have all distinct eigenvalues), this means that $\mtA$ and $\mtB$ can be written as a polynomial of $\mtS$,
% eq:polynomialOfS
\begin{equation} \label{eq:polynomialOfS}
    \mtA = p_{A}(\mtS) \quad , \quad \mtB = p_{B}(\mtS).
\end{equation}
%
Polynomials $p_{A}:\fdR \to \fdR$ and $p_{B}:\fdR \to \fdR$ are of degree at most $N-1$ \red{[Cite Cayley Hamilton]}.
Note that, when $\mtA$ and $\mtB$ can be written as a polynomial of $\mtS$, this implies that the dynamics evolving from $\vcx(t)$ to $\vcx(t+1)$ rely entirely on linear combinations carried out between components that share a connection, and hence, the system is considered distributed.
To see this, consider first the operation $\mtS \vcx(t)$ whose $i^{\text{th}}$ entry yields
% eq:graphShift
\begin{equation} \label{eq:graphShift}
    [\mtS \vcx(t)]_{i} = \sum_{j:(\lmv_{j},\lmv_{i}) \in \stE} [\mtS]_{ij} [\vcx(t)]_{j}.
\end{equation}
%
As it can be seen, due to the sparsity pattern of the GMD $\mtS$, the output of $\mtS\vcx(t)$ can be computed entirely as a linear combination of the states in neighboring nodes.
More generally, when considering polynomials, it is observed that $\mtS^{k}\vcx(t)$ is equivalent to exchanging $k$ times information with one-hop neighbors.
Therefore, if the system matrix $\mtA$ and the control matrix $\mtB$ are polynomials of $\mtS$, then the evolution of the system is computed entirely by means of exchanges with neighboring nodes.
Hence, Def.~\ref{def:distributedLinear} is a proper definition of distributed, linear systems.
Examples of such linear, distributed systems, include both discrete-time and continuous-time diffusions, solutions to the heat equation, among many others \red{[Add references]}.
